A Mel Spectrogram Enhancement Paradigm Based on CWT in Speech Synthesis

Acoustic features play an important role in improving the quality of the synthesised speech. Currently, the Mel spectrogram is a widely employed acoustic feature in most acoustic models. However, due to the fine-grained loss caused by its Fourier transform process, the clarity of speech synthesised by Mel spectrogram is compromised in mutant signals. In order to obtain a more detailed Mel spectrogram, we propose a Mel spectrogram enhancement paradigm based on the continuous wavelet transform (CWT). This paradigm introduces an additional task: a more detailed wavelet spectrogram, which like the post-processing network takes as input the Mel spectrogram output by the decoder. We choose Tacotron2 and Fastspeech2 for experimental validation in order to test autoregressive (AR) and non-autoregressive (NAR) speech systems, respectively. The experimental results demonstrate that the speech synthesised using the model with the Mel spectrogram enhancement paradigm exhibits higher MOS, with an improvement of 0.14 and 0.09 compared to the baseline model, respectively. These findings provide some validation for the universality of the enhancement paradigm, as they demonstrate the success of the paradigm in different architectures.

==> Figure/fig.tex <==
\definecolor{qblue}{RGB}{68,114,196}
\definecolor{qpurple}{RGB}{187,161,203}
\definecolor{qgreen}{RGB}{112,173,71}
\definecolor{qorange}{RGB}{237,125,49}
\definecolor{qpink}{RGB}{225,97,210}
\definecolor{qred}{RGB}{255,99,71}
\definecolor{qyellow}{RGB}{255,192,0}
\definecolor{sgreen}{RGB}{197,224,180}
\definecolor{syellow}{RGB}{255,230,153}
\definecolor{sblack}{RGB}{242,242,242}
\definecolor{backyellow}{RGB}{251,232,218}
\definecolor{backgreen}{RGB}{229,241,221}
\definecolor{backblue}{RGB}{189,215,238}
\begin{figure*}
    \centering
    \tikzstyle{textonly} = [font=\scriptsize,align=center]
    \tikzstyle{sublayer} = [rectangle,draw,minimum width=2.5cm,rounded corners=2.5pt,align=left,inner sep=1pt,minimum height=0.4cm,font=\scriptsize]
%%%    \tikzstyle{background} = [rectangle,rounded corners=3pt,minimum width=3.5cm,minimum height=3cm,font=\footnotesize,align=center];
%%%    \tikzstyle{arrow} = [font=\Large,align=center];
   \begin{tikzpicture}
    \node[sublayer,fill=white!70,draw=black,thick](simulst) at (0,0) {SimulST};
    %%%segmengpolicy
    \node[sublayer,fill=qorange!30,draw=qorange,thick,align=center,minimum width=3.3cm](segment) at ([yshift=3.3cm,xshift=2.3cm]simulst.east) {Segmentation Stategy};
    \node[sublayer,fill=qorange!30,draw=qorange,thick](fixed-length) at ([yshift=0.55cm,xshift=2cm]segment.east) {Fixed-length};
    \node[sublayer,fill=qorange!30,draw=qorange,thick](wordbd) at ([yshift=0cm,xshift=2cm]segment.east) {Word-based};
    \node[sublayer,fill=qorange!30,draw=qorange,thick](adaseg) at ([yshift=-0.55cm,xshift=2cm]segment.east) {Adaptive Segmentation};
    \node[sublayer,minimum width=4.3cm,dashed,draw=qorange,thick,fill=qorange!10]at([xshift=2.55cm]wordbd.east){Processing long-form speech inputs};
    %%%rwpolicy  exploring future research directions
    \node[sublayer,fill=qgreen!30,draw=qgreen,thick,minimum width=3.3cm](rwpolicy) at ([yshift=0.75cm,xshift=2.3cm]simulst.east) {Simul Read-Write Policy};
    \node[sublayer,fill=qgreen!30,draw=qgreen,thick](rwfixed) at ([yshift=0.85cm,xshift=2cm]rwpolicy.east) {Fixed};
    \node[sublayer,fill=qgreen!30,draw=qgreen,thick](waitk) at ([xshift=2cm]rwfixed.east) {Wait-\textit{k} Stride-\textit{n}} ;
    \node[sublayer,fill=qgreen!30,draw=qgreen,thick](waitkstride) at ([xshift=2cm,yshift=-0.55cm]rwfixed.east) {Wait-(\textit{k, s, n})};
    \node[sublayer,fill=qgreen!30,draw=qgreen,thick](waitksn) at ([xshift=2cm,yshift=0.55cm]rwfixed.east) {Wait-\textit{k}};
    \node[sublayer,fill=qgreen!30,draw=qgreen,thick](flexible) at ([yshift=-0.85cm,xshift=2cm]rwpolicy.east) {Flexible};      
    \node[sublayer,fill=qgreen!30,draw=qgreen,thick](aed) at ([yshift=0.55cm,xshift=2cm]flexible.east) {Attn-based Enc-Dec};  
    \node[sublayer,fill=qgreen!30,draw=qgreen,thick](o2o) at ([yshift=-0.55cm,xshift=2cm]flexible.east) {Offline-to-Simul};  
    \node[sublayer,fill=qgreen!30,draw=qgreen,thick](trans) at ([xshift=2cm]flexible.east) {Transducer};
    \node[sublayer,minimum width=4cm,dashed,draw=qgreen,thick,fill=qgreen!10]at([xshift=2.3cm,yshift=0.45cm]aed.east){Satisfying real-time requirements};
    %%%evaluation
    \node[sublayer,fill=qyellow!30,draw=qyellow,thick,minimum width=3.3cm](ql) at ([yshift=-1.55cm,xshift=2.3cm]simulst.east) {Evaluation Metrics};
    \node[sublayer,fill=qyellow!30,draw=qyellow,thick](eval) at ([yshift=0.3cm,xshift=2cm]ql.east) {Quality-based Metrics};
    \node[sublayer,fill=qyellow!30,draw=qyellow,thick](trade) at ([yshift=-0.3cm,xshift=2cm]ql.east) {Latency-based Metrics};
    \node[sublayer,minimum width=4.3cm,dashed,draw=qyellow,thick,fill=qyellow!10]at([xshift=2.55cm,yshift=-0.25cm]eval.east){Balancing quality and latency trade-offs};
    %%%datasacrity
    \node[sublayer,fill=qblue!30,draw=qblue,thick,minimum width=3.3cm](ds) at ([yshift=-2.72cm,xshift=2.3cm]simulst.east) {Augmented Training Methods};
    \node[sublayer,fill=qblue!30,draw=qblue,thick](mtasks) at ([yshift=0.3cm,xshift=2cm]ds.east) {Data Augmentation};
    \node[sublayer,fill=qblue!30,draw=qblue,thick](da) at ([yshift=-0.3cm,xshift=2cm]ds.east) {Multi-task Learning};
    \node[sublayer,minimum width=4.3cm,dashed,draw=qblue,thick,fill=qblue!10]at([xshift=2.55cm,yshift=-0.25cm]mtasks.east){Addressing data scarcity issues};
    %%%future
    %\node[sublayer,fill=qyellow!30,draw=qyellow,thick,minimum width=3.3cm](future) at ([yshift=-2cm,xshift=2cm]simulst.east) {Future Work};
    %\node[sublayer,fill=qyellow!30,draw=qyellow,thick](llm) at ([yshift=0.25cm,xshift=2cm]future.east) {Multilingual};
    %\node[sublayer,fill=qyellow!30,draw=qyellow,thick](multi) at ([yshift=-0.25cm,xshift=2cm]future.east) {Combining With LLM};

%%%st2other lines
\draw[-,thick](simulst.east)--([xshift=0.375cm]simulst.east)--([yshift=3.3cm,xshift=0.375cm]simulst.east)--(segment.west);
\draw[-,thick](simulst.east)--([xshift=0.375cm]simulst.east)--([yshift=0.75cm,xshift=0.375cm]simulst.east)--(rwpolicy.west);
\draw[-,thick](simulst.east)--([xshift=0.375cm]simulst.east)--([yshift=-1.55cm,xshift=0.375cm]simulst.east)--(ql.west);
\draw[-,thick](simulst.east)--([xshift=0.375cm]simulst.east)--([yshift=-2.72cm,xshift=0.375cm]simulst.east)--(ds.west);
%\draw[-,thick](simulst.east)--([xshift=0.375cm]simulst.east)--([yshift=-2cm,xshift=0.375cm]simulst.east)--(future.west);

%%%segments lines
\draw[-,thick](segment.east)--([xshift=0.375cm]segment.east)--([yshift=0.55cm,xshift=0.375cm]segment.east)--(fixed-length.west);
\draw[-,thick](segment.east)--([xshift=0.375cm]segment.east)--([yshift=-0.55cm,xshift=0.375cm]segment.east)--(adaseg.west);
\draw[-,thick](segment.east)--(wordbd.west);

%%%rw lines
\draw[-,thick](rwpolicy.east)--([xshift=0.375cm]rwpolicy.east)--([yshift=0.85cm,xshift=0.37cm]rwpolicy.east)--(rwfixed.west);
\draw[-,thick](rwfixed.east)--(waitk.west);
\draw[-,thick](rwfixed.east)--([xshift=0.375cm]rwfixed.east)--([yshift=-0.55cm,xshift=0.37cm]rwfixed.east)--(waitkstride.west);
\draw[-,thick](rwfixed.east)--([xshift=0.375cm]rwfixed.east)--([yshift=0.55cm,xshift=0.37cm]rwfixed.east)--(waitksn.west);

\draw[-,thick](rwpolicy.east)--([xshift=0.375cm]rwpolicy.east)--([yshift=-0.85cm,xshift=0.37cm]rwpolicy.east)--(flexible.west);
\draw[-,thick](flexible.east)--([xshift=0.375cm]flexible.east)--([yshift=0.55cm,xshift=0.375cm]flexible.east)--(aed.west);
\draw[-,thick](flexible.east)--(trans.west);
\draw[-,thick](flexible.east)--([xshift=0.375cm]flexible.east)--([yshift=-0.55cm,xshift=0.375cm]flexible.east)--(o2o.west);

%%%evaluation
\draw[-,thick](ql.east)--([xshift=0.375cm]ql.east)--([yshift=0.3cm,xshift=0.375cm]ql.east)--(eval.west);
\draw[-,thick](ql.east)--([xshift=0.375cm]ql.east)--([yshift=-0.3cm,xshift=0.375cm]ql.east)--(trade.west);

%%%data scarity
\draw[-,thick](ds.east)--([xshift=0.375cm]ds.east)--([yshift=0.3cm,xshift=0.375cm]ds.east)--(mtasks.west);
\draw[-,thick](ds.east)--([xshift=0.375cm]ds.east)--([yshift=-0.3cm,xshift=0.375cm]ds.east)--(da.west);

%%%future
%\draw[-,thick](future.east)--([xshift=0.375cm]future.east)--([yshift=0.25cm,xshift=0.375cm]future.east)--(llm.west);
%\draw[-,thick](future.east)--([xshift=0.375cm]future.east)--([yshift=-0.25cm,xshift=0.375cm]future.east)--(multi.west);
    
%%%% subfig1
\end{tikzpicture}
\caption{Key challenges to address in the task of SimulST and their corresponding solutions.}
\label{taxonomy}
\end{figure*}
